Beyond Grids: Exploring Elastic Input Sampling for Vision Transformers

Vision transformers have excelled in various computer vision tasks but mostly rely on rigid input sampling using a fixed-size grid of patches. It limits their applicability in real-world problems, such as active visual exploration, where patches have various scales and positions. Our paper addresses this limitation by formalizing the concept of input elasticity for vision transformers and introducing an evaluation protocol for measuring this elasticity. Moreover, we propose modifications to the transformer architecture and training regime, which increase its elasticity. Through extensive experimentation, we spotlight opportunities and challenges associated with such architecture.

==> figures/ave.tex <==
\begin{table}[t]
\caption{\textbf{Active visual exploration results:} We evaluate the performance of ElasticViT with MAE-like decoder head compared to standard MAE in active visual exploration scene reconstruction task performed by the AME algorithm. The metric is root mean squared error (RMSE; lower is better) and the dataset is ImageNet-1k. Our method outperforms competitive solutions.}
\label{tab:ame}
\begin{center}
\begin{small}
\vspace{-.2cm}
\begin{tabular}{l@{\hskip20pt}l}
\toprule
Method & RMSE \\
\midrule
MAE + AME & 30.5  \\
\textbf{ElasticMAE + AME (dual resolution)} & 25.95 \\
\textbf{ElasticMAE + AME (quad tree)} & \textbf{23.2}  \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\end{table}
